Enhancing Patient-Centric Communication: Leveraging LLMs to Simulate Patient Perspectives

Large Language Models (LLMs) have demonstrated impressive capabilities in role-playing scenarios, particularly in simulating domain-specific experts using tailored prompts. This ability enables LLMs to adopt the persona of individuals with specific backgrounds, offering a cost-effective and efficient alternative to traditional, resource-intensive user studies. By mimicking human behavior, LLMs can anticipate responses based on concrete demographic or professional profiles. In this paper, we evaluate the effectiveness of LLMs in simulating individuals with diverse backgrounds and analyze the consistency of these simulated behaviors compared to real-world outcomes. In particular, we explore the potential of LLMs to interpret and respond to discharge summaries provided to patients leaving the Intensive Care Unit (ICU). We evaluate and compare with human responses the comprehensibility of discharge summaries among individuals with varying educational backgrounds, using this analysis to assess the strengths and limitations of LLM-driven simulations. Notably, when LLMs are primed with educational background information, they deliver accurate and actionable medical guidance 88% of the time. However, when other information is provided, performance significantly drops, falling below random chance levels. This preliminary study shows the potential benefits and pitfalls of automatically generating patient-specific health information from diverse populations. While LLMs show promise in simulating health personas, our results highlight critical gaps that must be addressed before they can be reliably used in clinical settings. Our findings suggest that a straightforward query-response model could outperform a more tailored approach in delivering health information. This is a crucial first step in understanding how LLMs can be optimized for personalized health communication while maintaining accuracy.

==> scope_statement.tex <==
Authors should read the call for papers carefully which have been updated from last year's call. In particular, please ensure
The paper is appropriate for CSCW (see the Section "Paper Guidelines Regarding Scope") in the call for papers.
You understand the various criteria for desk / quick reject in the call for papers.
Due to the quantity of papers we receive, we must strictly and consistently enforce the stated policies in our call for papers. Below, please answer the two questions (1-4 sentences in total):

How does your work build upon, bridge, discuss, or cite prior CSCW work in a significant manner?
How are the results of your work useful for thinking about the design of computing technologies to support cooperative/collaborative work or social interactions?

1. Our paper builds upon and contributes to CSCW by focusing on **domain-specific social, cooperative, and collaborative applications** within healthcare. Zhu et al. [1] from CSCW ’23 emphasized the importance of leveraging large language models (LLMs) to support human problem-solving, especially in processing associated knowledge. 

%noting their potential not only for processing human language but also for managing associated knowledge. 
Additionally, the CSCW ’19 workshop identified critical challenges and opportunities in advancing human-AI collaboration, particularly in healthcare settings [2].

% Our work builds on this foundation by enhancing patient-centered LLMs to provide personalized healthcare support. Specifically, we aim to simplify clinical processes by assisting in diagnosis and documentation analysis, contributing to more streamlined and supportive healthcare services.

We draw from prior CSCW work on cooperative information-sharing practices to explore how LLMs can enhance patient-provider communication, particularly for diverse and underserved populations. This approach provides new insights for the CSCW community on using technology to facilitate social and collaborative interactions in healthcare settings.
	
2.	The results of our study underscore both the effectiveness and challenges of LLM personalization, revealing biases and misalignments in tailored responses. We observed notable discrepancies in LLM output accuracy when correlated with factors like user education level and gender. These insights are valuable for the design of computing technologies that seek to support collaborative healthcare interactions, emphasizing the importance of addressing these biases to achieve more equitable and reliable AI-driven assistance in clinical settings.

Final submission:

Our paper builds upon and contributes to CSCW by focusing on **domain-specific social, cooperative, and collaborative applications** within healthcare. Zhu et al. [1] from CSCW ’23 emphasized the importance of leveraging large language models (LLMs) to support human problem-solving, especially in processing associated knowledge. Additionally, the CSCW ’19 workshop identified critical challenges and opportunities in advancing human-AI collaboration, particularly in healthcare settings[2]. We draw from prior CSCW work on cooperative information-sharing practices to explore how LLMs can enhance patient-provider communication, particularly for diverse and underserved populations. This approach provides new insights for the CSCW community on using technology to facilitate social and collaborative interactions in healthcare settings.

[1] Qingxiaoyang Zhu and Hao-Chuan Wang. 2023. Leveraging Large Language Model as Support for Human Problem Solving: An Exploration of Its Appropriation and Impact. In Companion Publication of the 2023 Conference on Computer Supported Cooperative Work and Social Computing (CSCW '23 Companion). Association for Computing Machinery, New York, NY, USA, 333–337. https://doi.org/10.1145/3584931.3606965

[2] Sun Young Park, Pei-Yi Kuo, Andrea Barbarin, Elizabeth Kaziunas, Astrid Chow, Karandeep Singh, Lauren Wilcox, and Walter S. Lasecki. 2019. Identifying Challenges and Opportunities in Human-AI Collaboration in Healthcare. In Companion Publication of the 2019 Conference on Computer Supported Cooperative Work and Social Computing (CSCW '19 Companion). Association for Computing Machinery, New York, NY, USA, 506–510. https://doi.org/10.1145/3311957.3359433 
